A new temperature evolution equation that enforces thermodynamic vapour-liquid equilibrium in multiphase flows -- application to CO2 modeling

This work presents a novel framework for numerically simulating the depressurization of tanks and pipelines containing carbon dioxide (CO2). The framework focuses on efficient solution strategies for the coupled system of fluid flow equations and thermodynamic constraints. A key contribution lies in proposing a new set of equations for phase equilibrium calculations which simplifies the traditional vapor-liquid equilibrium (VLE) calculations for two-phase CO2 mixtures. The first major novelty resides in the reduction of the conventional four-equation VLE system to a single equation, enabling efficient solution using a non-linear solver. This significantly reduces computational cost compared to traditional methods. Furthermore, a second novelty is introduced by deriving an ordinary differential equation (ODE) directly from the UV-Flash equation. This ODE can be integrated alongside the governing fluid flow equations, offering a computationally efficient approach for simulating depressurization processes.

==> metadata/authors.tex <==
\author[a,b]{P. Kumar\footnote{Corresponding author: pardeep@cwi.nl}}
\author[a,c]{B. Sanderse}
\author[d]{P.I. Rosen Esquivel}
% \author[b,d]{R. A. W. M. Henkes}

% \author{
%     Pardeep Kumar$^{a,b}$ \and
%     Benjamin Sanderse$^{a,c}$ \and
%     Patricio Rosen Esquivel$^{d}$ \and
%     Ruud Henkes$^{b,d}$
% }

\affil[a]{{\small Centrum Wiskunde \& Informatica (CWI), Amsterdam, The Netherlands}}
\affil[b]{{\small Delft University of Technology, Delft, The Netherlands}}
\affil[c]{{\small Eindhoven University of Technology, Eindhoven, The Netherlands}}
\affil[d]{{\small Shell Projects and Technology, The Netherlands}}

\date{\today}

==> metadata/highlights.tex <==
\section{Highlights}

\begin{enumerate}
    \item Reduction of two-phase UV-Flash from four equations to a single equation.
    \item Proposed a novel temperature evolution equation consistent with the single-equation flash.
    \item Achieved significant computational performance improvement.
    \item Application to modeling depressurization in tanks and pipelines filled with \coo.
\end{enumerate}




==> metadata/refs_manual.tex <==
\begin{thebibliography}{10}

\bibitem{noauthor_iea_2023}
{IEA} (2023), {Energy} {Technology} {Perspectives}, {IEA}, {Paris}
  https://www.iea.org/reports/energy- technology-perspectives-2023, {License}:
  {CC} {BY} 4.0.
\newblock Technical report, 2023.

\bibitem{ascher_computer_1998}
U.~M. Ascher and L.~R. Petzold.
\newblock {\em Computer methods for ordinary differential equations and
  differential-algebraic equations}.
\newblock Society for Industrial and Applied Mathematics, Philadelphia, 1998.

\bibitem{bell_efficient_2021}
I.~H. Bell and B.~K. Alpert.
\newblock Efficient and {Precise} {Representation} of {Pure} {Fluid} {Phase}
  {Equilibria} with {Chebyshev} {Expansions}.
\newblock {\em International Journal of Thermophysics}, 42(5):75, May 2021.

\bibitem{bruce_stewart_two-phase_1984}
H.~Bruce~Stewart and B.~Wendroff.
\newblock Two-phase flow: {Models} and methods.
\newblock {\em Journal of Computational Physics}, 56(3):363--409, Dec. 1984.

\bibitem{castier_solution_2009}
M.~Castier.
\newblock Solution of the isochoric–isoenergetic flash problem by direct
  entropy maximization.
\newblock {\em Fluid Phase Equilibria}, 276(1):7--17, Feb. 2009.

\bibitem{clerc_numerical_2000}
C.~Clerc.
\newblock Numerical {Simulation} of the {Homogeneous} {Equilibrium} {Model} for
  {Two}-{Phase} {Flows}, 2000.

\bibitem{giljarhus_solution_2012}
K.~E.~T. Giljarhus, S.~T. Munkejord, and G.~Skaugen.
\newblock Solution of the {Span}-{Wagner} equation of state using a
  density-energy state function for fluid-dynamic simulation of carbon dioxide.
\newblock In {\em Industrial and {Engineering} {Chemistry} {Research}},
  volume~51, pages 1006--1014. Journal of Fluids and Structures, Jan. 2012.
\newblock Issue: 2 ISSN: 08885885.

\bibitem{hairer_numerical_1989}
E.~Hairer, C.~Lubich, and M.~Roche.
\newblock {\em The numerical solution of differential-algebraic systems by
  {Runge}-{Kutta} methods}.
\newblock Number 1409 in Lecture notes in mathematics. Springer, Berlin
  Heidelberg, 1989.

\bibitem{hairer_geometric_2006}
E.~Hairer, G.~Wanner, and C.~Lubich.
\newblock {\em Geometric {Numerical} {Integration}}, volume~31 of {\em Springer
  {Series} in {Computational} {Mathematics}}.
\newblock Springer-Verlag, Berlin/Heidelberg, 2006.

\bibitem{hammer_method_2013}
M.~Hammer, A.~Ervik, and S.~T. Munkejord.
\newblock Method {Using} a {Density}–{Energy} {State} {Function} with a
  {Reference} {Equation} of {State} for {Fluid}-{Dynamics} {Simulation} of
  {Vapor}–{Liquid}–{Solid} {Carbon} {Dioxide}.
\newblock {\em Industrial \& Engineering Chemistry Research},
  52(29):9965--9978, July 2013.

\bibitem{hammer_method_2014}
M.~Hammer and A.~Morin.
\newblock A method for simulating two-phase pipe flow with real equations of
  state.
\newblock {\em Computers \& Fluids}, 100:45--58, Sept. 2014.

\bibitem{ishii_thermo-fluid_2011}
M.~Ishii and T.~Hibiki.
\newblock {\em Thermo-fluid dynamics of two-phase flow}.
\newblock Springer, New York, 2nd ed edition, 2011.
\newblock OCLC: ocn690084123.

\bibitem{lund_depressurization_2011}
H.~Lund, T.~Flåtten, and S.~Tollak~Munkejord.
\newblock Depressurization of carbon dioxide in pipelines–{Models} and
  methods.
\newblock {\em Energy Procedia}, 4:2984--2991, 2011.

\bibitem{menikoff_riemann_1989}
R.~Menikoff and B.~J. Plohr.
\newblock The {Riemann} problem for fluid flow of real materials.
\newblock {\em Reviews of Modern Physics}, 61(1):75--130, Jan. 1989.

\bibitem{michelsen_isothermal_nodate}
Michelsen.
\newblock {THE} {ISOTHERMAL} {FLASH} {PROBLEM}. {PART} {II}. {PHASE}-{SPLIT}
  {CALCULATION}.

\bibitem{michelsen_state_1999}
M.~L. Michelsen.
\newblock State function based flash specifications.
\newblock {\em Fluid Phase Equilibria}, 158-160:617--626, June 1999.

\bibitem{michelsen_thermodynamic_2007}
M.~L. Michelsen and J.~M. Mollerup.
\newblock {\em Thermodynamic models : fundamentals \& computational aspects}.
\newblock Tie-Line Publications, 2007.

\bibitem{munkejord_depressurization_2015}
S.~T. Munkejord and M.~Hammer.
\newblock Depressurization of {CO2}-rich mixtures in pipes: {Two}-phase flow
  modelling and comparison with experiments.
\newblock {\em International Journal of Greenhouse Gas Control}, 37:398--411,
  June 2015.
\newblock Publisher: Elsevier Ltd.

\bibitem{munkejord_co2_2016}
S.~T. Munkejord, M.~Hammer, and S.~W. Løvseth.
\newblock {CO2} transport: {Data} and models – {A} review.
\newblock {\em Applied Energy}, 169:499--523, May 2016.

\bibitem{saha_isoenergetic-isochoric_1997}
S.~Saha and J.~J. Carroll.
\newblock The isoenergetic-isochoric flash.
\newblock {\em Fluid Phase Equilibria}, 138(1-2):23--41, Nov. 1997.

\bibitem{saurel_modelling_2008}
R.~Saurel, F.~Petitpas, and R.~Abgrall.
\newblock Modelling phase transition in metastable liquids: {Application} to
  cavitating and flashing flows.
\newblock {\em Journal of Fluid Mechanics}, 607:313--350, July 2008.
\newblock Publisher: Cambridge University Press.

\bibitem{sirianni_explicit_2024}
G.~Sirianni, A.~Guardone, B.~Re, and R.~Abgrall.
\newblock An {Explicit} {Primitive} {Conservative} {Solver} for the {Euler}
  {Equations} with {Arbitrary} {Equation} of {State}, Apr. 2024.
\newblock arXiv:2404.07710 [cs, math].

\bibitem{smejkal_phase_2017}
T.~Smejkal and J.~Mikyška.
\newblock Phase stability testing and phase equilibrium calculation at
  specified internal energy, volume, and moles.
\newblock {\em Fluid Phase Equilibria}, 431:82--96, Jan. 2017.

\bibitem{span_new_1996}
R.~Span and W.~Wagner.
\newblock A {New} {Equation} of {State} for {Carbon} {Dioxide} {Covering} the
  {Fluid} {Region} from the {Triple}-{Point} {Temperature} to 1100 {K} at
  {Pressures} up to 800 {MPa}.
\newblock {\em Journal of Physical and Chemical Reference Data},
  25(6):1509--1596, Nov. 1996.

\bibitem{toro_riemann_2009}
E.~F. Toro.
\newblock {\em Riemann {Solvers} and {Numerical} {Methods} for {Fluid}
  {Dynamics}}.
\newblock 2009.

\bibitem{toumi_weak_1991}
I.~Toumi.
\newblock A weak formulation of {Roe} approximate {Riemann} {Solver}.
\newblock 1991.

\bibitem{toumi_approximate_1999}
I.~Toumi, A.~Kumbaro, and H.~Pailler.
\newblock Approximate {Riemann} solvers and flux vector splitting schemes for
  two-phase flow.
\newblock Technical Report CEA-R-5849(E), 1999.

\end{thebibliography}


==> paper/sections/reproducibility.tex <==
% \section{Reproducibility statement} \label{sec:reproducibility}
\section*{Software and reproducibility statement}

The source code is not open.

